Dimensioning of V2X Services in 5G Networks through Forecast-based Scaling

With the increasing adoption of intelligent transportation systems and the upcoming era of autonomous vehicles, vehicular services (such as, remote driving, cooperative awareness, and hazard warning) will face an ever changing and dynamic environment. Traffic flows on the roads is a critical condition for these services and, therefore, it is of paramount importance to forecast how they will evolve over time. By knowing future events (such as, traffic jams), vehicular services can be dimensioned in an on-demand fashion in order to minimize Service Level Agreements (SLAs) violations, thus reducing the chances of car accidents. This research departs from an evaluation of traditional time-series techniques with recent Machine Learning (ML)-based solutions to forecast traffic flows in the roads of Torino (Italy). Given the accuracy of the selected forecasting techniques, a forecast-based scaling algorithm is proposed and evaluated over a set of dimensioning experiments of three distinct vehicular services with strict latency requirements. Results show that the proposed scaling algorithm enables resource savings of up to a 5% at the cost of incurring in an increase of less than 0.4% of latency violations.

==> dataset.tex <==
\section{Torino road traffic dataset}
\label{sec:dataset}
This section presents the real road traffic dataset utilized in this paper. The dataset contains information of Torino city
traffic flows, with measurements from more than 
100 road probes reporting their
location, traffic flow, and vehicles speed.

The data is gathered by using S.I.MO.NE protocol~\cite{simone},
and exposed via an API\footnote{\url{http://opendata.5t.torino.it/get_fdt}}. Thus, probes' measurements are fetched every 5 minutes,
and gathered in a common eXtensible Markup Language (XML) file.
Each entry in the XML file represents the measurements
that a probe aggregates every 5 minutes, containing fields~\cite[Table 8]{simone-xml} such as: \emph{(i)} probes'
latitude and longitude; \emph{(ii)} their identification codes,
\emph{(iii)} their offsets along the road; \emph{(iv)} the road names;
\emph{(v)} average speed of vehicles; \emph{(vi)} vehicles flow, i.e.,
vehicles per hour; \emph{(vii)} measurements accuracy; and
\emph{(viii)} timestamp.
In this work, all entries of the gathered XML files have been collapsed in a Comma-Separated Values (CSV) dataset with samples from 28/01/2020 to 25/03/2020.

Not every road probe reports data with the same frequency. Indeed, some of them suddenly stop reporting measurements during the night, or even worse, in the middle
of rush hours.
Such behavior might be caused by errors in
the probes' hardware, or just by decisions of Torino city
Mobility Central.
Thus, the collapsed CSV dataset required of some filtering
to remove spurious probes, i.e., probes reporting less
than an 80\% of the measurements they should have reported
(one every 5 minutes).
Among the 116 road probes present in the dataset, 24 of
them did not satisfied such requirement and were removed
from the CSV dataset.

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{img/traffic-drop.pdf}
    \caption{Impact of COVID-19 in Torino traffic flow. The figure plots the sum of all road probes' traffic flows.}
    \label{fig:impact-COVID-19}
\end{figure}


Even after pruning spurious road probes, the dataset
still had probes that spent up to a 20\% of the time
without reporting data.
Thus, the dataset was sanitized to fill those missing values
with the last reported probe measurement.
%Sanitizing the entire CSV dataset turned out to be computationally intensive - an Intel Core i7-5600U CPU @ 2.60GHz spent 28h to just sanitize the 41\% of the dataset. To speed up the sanitation of 1,545,553 probe measurements, the 28/01/2020 to 25/03/2020 time span was split into ten intervals, and each interval was sanitized in parallel by x10 Intel Xeon CPU E5-2670 0 @ 2.60GHz. As a result, all the dataset were sanitized in around 3h30min.
However, this first sanitation sweep was not 
sufficient, because there were still missing
timestamps.
The first sweep just considered as timestamps
those reported by any road probe of the dataset,
hoping that every time instant would be
present in the reported information.
But, it happened that for some instants of
time (e.g., at 2020-02-15 at 04:25) no road probe
reported data (this might be because
the company
managing road probes might turn them off
in the wee hours of the morning).
Thus, the first sanitation
sweep missed such values.
To fix the issue, a second sanitation sweep
looked for those missing timestamps all
over the dataset, which are filled with the
most recent information.
%The process took ~6:40~min. in a single Intel Xeon CPU E5-2670 0 @ 2.60GHz CPU.


By the time the dataset was collected,
the COVID-19 pandemic struck northern
Italy, and, consequently, there was a significant drop of
the flow of vehicles in the city of Torino.
More precisely, on February 23\textsuperscript{rd} the region of Piemonte (where Torino is)
applied a Health Ministry
order~\cite{23feb-measurements} that
temporarily suspended teaching activities
in the region.
And under the pandemic expansion,
the 4\textsuperscript{th} of March a new
decree~\cite{4mar-measurements} extended 
the restrictions until the 15\textsuperscript{th}
of March.
But it is not until the 8\textsuperscript{th}
of March when the vehicles per day show a
significant drop in Torino city (see
Figure~\ref{fig:impact-COVID-19}).
That day the
government imposed a
lockdown~\cite{8mar-measurements} in other
northern regions of Italy that did not affect
Torino, which did not experienced
lockdown until the 11\textsuperscript{th} of
March~\cite{11mar-measurements}.
But, even though Torino was not in lockdown
by the 8\textsuperscript{th} of March,
the traffic decrease after then
was more significant than the decrease
experienced after the 23\textsuperscript{rd} of
February.
Figure~\ref{fig:impact-COVID-19} shows a traffic
decrease of a 9.82\% from the 27\textsuperscript{th} of February to the 8\textsuperscript{th} of March,
whilst after
the 8\textsuperscript{th} of March the decrease dropped down to
57.53\%.

COVID-19 impact on the traffic of Torino is
a relevant factor to consider for the
forecasting techniques presented in
Section~\ref{sec:techniques}, as it allowed to assess how each technique is able to adapt to changing patterns.
Thus, and based in the average traffic decrease,
the remaining of this paper considers the
8\textsuperscript{th} of March as the date
splitting the dataset into non-COVID-19 (before), and
COVID-19 (after) periods.

==> forecastingtechniques.tex <==
\section{Forecasting techniques - UC3M+NBL+SSSA}
\label{sec:techniques}
describe the SoA techniques we've used, and how we
implemented online training on each of them;\\


This section describes the different forecasting techniques such as Simple Exponential Smoothing (SES), Double Exponential Smoothing (DES), Triple Exponential Smoothing (TES), and Hierarchical Temporal Memory (HTM). These considered forecasting techniques are compared to ML-based techniques such as Long Short-Term Memory (LSTM), and Gated Recurrent Units (GRUs). 

\subsection{Simple Exponential Smoothing \text{(SES)}} 

\subsection{Double Exponential Smoothing \text{(DES)}} 
DES is a forecasting technique based on time series analysis. DES uses a smoothing $S_t$ time scale with a level factor $\alpha \in [0, 1]$, and trend smoothing $T_t$ with a trend factor $\beta \in [0, 1]$ as described in Eqs.~(\ref{e:deslt}) and (\ref{e:destt}). The smoothing time scale is obtained based on the previous experienced time interval value of smoothing $S_{t-1}$ and trend $T_{t-1}$. Note that in Eq.~(\ref{e:deslt}), the current value of time series (i.e., $f_t$) is used to predict the flow values.
\begin{IEEEeqnarray}{rCl}
L_t &= & \alpha \cdot f_t + (1-\alpha) \cdot (L_{t-1} + T_{t-1})
\label{e:deslt}
\end{IEEEeqnarray}
\vspace{-2.5em}
\begin{IEEEeqnarray}{rCl}
T_t &= & \beta \cdot (L_t - L_{t-1}) + (1-\beta) \cdot T_{t-1}.
\label{e:destt}
%\vspace{-1.2em}
\end{IEEEeqnarray}
The following Eq. (\ref{e:desyt}) is used to obtained k-steps ahead (namely \emph{lead time}) forecast ${y}_{t+k}$ in DES:
\begin{IEEEeqnarray}{rCl}
 \widehat{f}_{t+k} &= & L_t + k \cdot T_{t}.
\label{e:desyt}
%\vspace{-1.2em}
\end{IEEEeqnarray}

\subsection{Triple Exponential Smoothing \text{(TES)}} 

TES in another time series analysis technique. As shown in Eqs.~(\ref{e:teslt})-(\ref{e:tesst}), TES exploits three different forecasting factors such as \emph{level}, \emph{trend} and \emph{seasonality}. Here, $\widehat{y}_{t+k}$ represents the forecast at time $t + k$ given all the data points up to time $t$, and the seasonality constant $s$ (i.e., the number of observations per season). TES can be performed in two ways, namely \emph{additive} and \emph{multiplicative} techniques, depending on the seasonality effect. Note that the following equations are defined based on the \emph{additive} technique:
\begin{IEEEeqnarray}{rCl}
L_t &= & \alpha \cdot (y_t - S_{t-s}) + (1-\alpha) \cdot (L_{t-1} + T_{t-1})
\label{e:teslt}
\end{IEEEeqnarray}
\vspace{-2.5em}
\begin{IEEEeqnarray}{rCl}
T_t &= & \beta \cdot (L_t - L_{t-1}) + (1-\beta) \cdot T_{t-1}
\label{e:testt}
\end{IEEEeqnarray}
\vspace{-2.5em}
\begin{IEEEeqnarray}{rCl}
 S_t &= & \gamma \cdot (y_t - T_t) + (1-\gamma) \cdot S_{t-s}
\label{e:tesst}
\end{IEEEeqnarray}
\vspace{-2.5em}
\begin{IEEEeqnarray}{rCl}
 \widehat{y}_{t+k} &= & L_t + k \cdot T_{t} + S_{t+k-s},
\label{e:tesyt}
\end{IEEEeqnarray}

where s is the length of the seasonal cycle, for $\alpha \in [0,1]$, $\beta \in [0,1]$, and $\gamma \in [0,1]$. 

\subsection{Hierarchical Temporal Memory \text{(HTM)}} 

The core component of the HTM predictor \cite{Ahmad2017} is a temporal memory $M(.,.)$ consisting of a set of cells arranged in columns, where the cells can influence each other via synapses. During training the temporal memory is presented with a sequence of input sparse bit strings. For each sparse input bit string $s_t, \: t=0, 1, \ldots$ in the sequence, it produces an output sparse bit string $\hat{s}_{t,1} = M(s_t, \omega)$ (of the same length) that depends on the current value $\omega$ of the synapses and serves as a forecasting for the next sparse bit string $s_{n+1}$. The temporal memory can predict not only the next sparse bit string, but also the following ones by building upon consecutive forecasts, e.g., the forecast $k > 1$ time units in future is obtained via $\hat{s}_{t,k} = M(\hat{s}_{t,k-1}, \omega)$. Learning involves adjusting the synapses $\omega$ in such a way that the output bit strings $\hat{s}_{t,k} \: (k \leq 1)$ resemble the actual input bit strings $s_{t+k} \: (k \leq 1)$ as much as possible. In that way the temporal memory learns to predict the next sparse bit strings based on the patterns in the sequence of input bit string it saw. 

When being presented with a sequence of floating point values $f_t$ the HTM predictor first translates these floating point values in sparse bit strings via an encoder $s_t = E(f_t)$. Once the values of the sequence are encoded in bit strings by this encoder, the temporal memory learns to predict the sparse bit strings as described before.

Finally, the predicted bit strings need to be translated to floating point variables again, which is the job of a classifier. The classifier chooses as forecast $\hat{f}_{t,k}$, $k$ time slots in future, for the floating point value, the value for which the bit string it encodes to lies closest to the bit string predicted by the temporal memory, i.e., $E(\hat{f}_{t,k})$ closest to $\hat{s}_{t,k}$.  

Untrained the HTM predictor sets $\hat{s}_{t,k} = s_n$, which is equivalent to a sample-and-hold strategy that we use as benchmark. After training, the forecasts are more elaborate. 

In the experiments below we used a temporal memory of 2048 columns of 32 cells each and the encoder mapped floating point values in bit strings of 1020 bits of which only 21 where non-zero. We run through the training set once (and checked that running through it more did not have a beneficial effect) and then either stopped the learning process before running through the test set to obtain the "offline" results or continued training while running through the test set to obtain the "online" results. 

\subsection{Long Short-Term Memory \text{(LSTM)}} 



\subsection{Gated Recurrent Unit \text{(GRU)}} 

==> motivation.tex <==

%\section{Vehicular services \& scaling motivation}
\section{Motivation}
\label{sec:motivation}

Connected and automated vehicles (CAVs) represent one of the most significant transformations of the automobile industry, providing an opportunity to enhance monitoring of transportation network conditions, in order to improve safety and reduce pollution, energy consumption, and travel delays. 
5G systems are gaining traction as a viable technological solution, due to the ubiquity of the cellular infrastructure. Moreover, by ensuring ultra-low latency and ultra-high reliability communications under high-density and high-mobility conditions, 5G systems will enable Cellular Vehicle-to-Everything (C-V2X) communications.
 
The C-V2X technology has been designed by the Third Generation Partnership Project (3GPP) to allow vehicles to communicate with other vehicles (vehicle-to-vehicle, V2V), road users (vehicle-to-pedestrian, V2P), roadside infrastructure (vehicle-to-infrastructure, V2I), and cloud/edge servers (vehicle-to-network, V2N) \cite{3GPPV2X1}. The 3GPP specifies the Enhancement of 3GPP support for V2X services (eV2X) in the following four areas: \emph{(i)} Vehicles Platooning; \emph{(ii)} Advanced Driving; \emph{(iii)} Extended Sensors; and \emph{(iv)} Remote Driving \cite{3GPPV2X2}.  The European Telecommunication Standard Institute (ETSI) Multi-Access Edge Computing (MEC) group has also collected the corresponding requirements for MEC, by analyzing the relevant V2X use cases \cite{gr-mec022} pertaining to safety, convenience, advanced driving assistance and vulnerable road users. 

All aforementioned cases require process-intensive and low-latency, reliable computing and communication services. For example, remote driving applications require values of 99.999\% reliability and 5ms end-to-end (E2E) latency with a rate of 25Mbps and 1Mbps for the UL and DL respectively.

Such characteristics prohibit cloud-based solutions, due to the long delays to reach the cloud. An effective approach to address such requirements is to leverage the edge computing paradigm \cite{7488250}. Edge Computing provides a low-latency alternative to the cloud, moving computational resources to the edge, closer to where the data is being generated, processed, and most likely consumed. %To meet the resulting communication requirements. 
However, edge computing devices have limited processing resources. Therefore, careful resource scaling or (re)allocation is needed to meet both the computational and the latency requirements of vehicular applications.  Indicatively, in \cite{premsankar2018efficient}, the efficient placement of edge computing devices is addressed for vehicular applications in an urban scenario, by mapping the average number of vehicles in each cell to Central Processing Unit (CPU) demand. However, to tackle such resource allocation problem optimally over time or to scale resources cost-effectively, the evolution of the network traffic demand is needed per cell.

This paper compares different forecasting
techniques to forecast road traffic evolution over time.
The per-cell granularity is granted thanks to
per-road forecasts that use a Torino road traffic
dataset (see Section~\ref{sec:dataset}).
Traffic forecasts are later used to
dynamically scale-out the network slice  computational resources (at the edge), supporting the requirements for three different C-V2N use cases, drawn from the ETSI~\cite{gr-mec022}\cite{gs-mec022} and 3GPP\cite{3GPPV2X2} use case portfolio:

% Towards this direction, we employ road traffic prediction, using the Torino road traffic dataset described in section \ref{sec:dataset}, to dynamically scale-out the network slice  computational resources (at the edge), supporting the requirements for three different C-V2N use cases, drawn from the ETSI~\cite{gr-mec022}\cite{gs-mec022} and 3GPP\cite{3GPPV2X2} use case portfolio:


%\subsection{V2N services' requirements} % - 2-3 pag. - SSSA+UC3M+NBL}
%\label{sec:service-requirements}


%\reviewerone{The organization is not satisfying [referes to the whole paper];

%Why do you present the latency requirements so late in Section VII?}
%There exist multiple V2X (vehicle to everything) services which aim at improving different aspects of vehicular scenarios, from safety to traffic efficiency and also pure information \& entertainment~\cite{gr-mec022}\cite{gs-mec022}\cite{3GPPV2X2}. Among those, we focus on some V2N examples that pose strict requirements on latency:

\begin{itemize}

\item \textit{Remote Driving} to enable the remote operation of a vehicle by a remote driver or a cloud-based application. Different use case scenarios can benefit of such approach, ranging from the operation of vehicles that are located in dangerous environments, assistance of passengers that cannot drive by themselves, or support of autonomous vehicles that are in unexpected situations. Usually, the information exchanged between the V2X application in the vehicle and the V2X application server includes live video streams of on-board cameras and driving commands. These use cases can benefit from computational resources at the edge to locally process vehicle's information and compute the driving commands. Such applications require E2E latency below 5ms \cite{3GPPV2X2}.

\item \textit{Cooperative awareness} to improve traffic efficiency. This also encompasses multiple use cases, with the goal of improving overall traffic efficiency by sharing specific pieces of information and/or coordinating actions of several vehicles. Examples of these applications are lane change assistance, co-operative glare reduction, co-operative merging assistance, traffic light optimal speed advisory, etc.~\cite{tr-102}. These use cases benefit from computational resources at the edge, to collect, process and decide what information/command to distribute and to which vehicles. These applications typically require latency between 100ms and 500ms. 

\item \textit{Hazard warning} to share and distribute pieces of information for avoiding a risk (e.g., danger on a lane, intersection warning, collision avoidance) or minimizing the consequences of it (e.g., pre-configuration of seat-belts in preparation of an imminent accident). Computing resources at the edge can be used to extend the connected car cloud into the highly distributed mobile network environment. As described in~\cite{gs-mec022}, applications can be deployed on the edge to provide the roadside functionality: \emph{(i)} receiving local messages directly from the applications in the vehicles and the roadside sensors; \emph{(ii)} analyzing
them; and \emph{(iii)} propagating (with extremely low latency) hazard warnings and other latency-sensitive messages to other
cars in the area. If provided within very low and strict latency constraints, vehicles in the local vicinity of a dangerous situation receive data in a matter of milliseconds, allowing the driver to immediately adopt preventive actions (e.g. switch lanes, slow down or change his route). Depending on the type of event, the speed of the road and the traffic density, these applications require latency between 10 and 50ms~\cite{tr-102}.

\end{itemize}
